Eccentricity-Constrained CNN Training Reveals Adaptive Information Coding Around the Visual Field

In the primate visual system, center-preferring cortical populations have higher spatial resolution and overlap face- and word-selective regions while periphery-preferring populations have lower spatial resolution and overlap scene-selective regions. This "eccentricity bias" may reflect differential task-relevance: central vision may better support fine-grained tasks like face recognition and reading, while peripheral vision may better support scene understanding. To test whether eccentricity-dependent coding can emerge from natural experience, we used egocentric video and eye-tracking data from the Visual Experience Dataset (VEDB). We trained ResNet-18 models using contrastive learning (SimCLR) on frames modified to isolate different eccentricities (gaze-contingent fovea-only crops, periphery-only crops, and periphery-only crops with a NeuroFovea transform applied). We evaluated downstream task performance and model alignment with human fMRI data (Natural Scenes Dataset; encoding models). In-domain VEDB frame classification showed systematic differences between fovea- and periphery-only models across categories, indicating differential informativeness across tasks. On downstream classification, VEDB-pretrained models generalized better to scene categorization (Places365) than face recognition (VGGFace2), with fovea-only models stronger on both. Across visual cortex, VEDB-pretrained models matched neural predictivity of models trained on mid-sized non-egocentric datasets (ImageNet-100), suggesting egocentric data supports emergence of cortically-aligned representations. In scene-selective cortex (PPA, RSC), periphery-only models held a small but consistent advantage in explained variance over fovea-only models, suggesting these regions are aligned with peripheral statistics. Together, these results suggest egocentric experience may adaptively constrain cortical information processing.

==> tables/table_export_conditions.tex <==
\begin{table}[t]
\centering
\captionsetup{font=normalsize} % 10pt in a 10pt document

\caption{Summary Metrics for Pretraining and Linear Probes. SimCLR Top-1 is computed from the self-supervised contrastive objective and is not directly comparable to downstream classification. For downstream tasks, classifier checkpoints were selected by best validation Macro-F1. In-domain Top-1 accuracy is omitted because label imbalance across frames can make accuracy misleading; Macro-F1 is reported as the primary class-balanced metric. STL-10, ImageNet-100, and ImageNet-1K are treated as out-of-domain baselines because they were not pretrained on VEDB.}
\label{tab:linear_probe_summary}

\scriptsize
\setlength{\tabcolsep}{1.2pt}
\renewcommand{\arraystretch}{0.88}

\scalebox{1.00}{
\begin{tabular}{@{} p{1.25cm} p{1.65cm} r r r r @{}}
\toprule
\textbf{Task} & \textbf{Condition} & \textbf{Val Loss} & \textbf{Top-1 (\%)} & \textbf{Top-5 (\%)} & \textbf{Best Macro-F1 (\%)} \\
\midrule

\multirow{4}{*}{SimCLR}
  & Baseline    & 0.4331 & 87.60 & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} \\
  & Fovea-Gaze  & 0.3749 & 90.43 & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} \\
  & Periph-NF   & 0.4548 & 90.04 & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} \\
  & Periph      & 0.4545 & 89.26 & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} \\
\midrule

\multirow{6}{*}{In-Domain}
  & Baseline    & 0.9811 & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} & 42.17 \\
  & Fovea-Gaze  & 1.2031 & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} & 43.64 \\
  & Periph-NF   & 1.3090 & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} & 30.93 \\
  & Periph      & 1.0623 & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} & 36.56 \\
  & STL-10       & 1.6666 & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} & 25.41 \\
  & ImageNet-100 & 1.2342 & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} & 41.23 \\
  & ImageNet-1K & 0.9713 & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} & 43.33 \\
\midrule

\multirow{6}{*}{VGGFace2}
  & Baseline    & 7.8101 & 5.21  & 11.73 & 3.26 \\
  & Fovea-Gaze  & 7.9104 & 4.58  & 10.76 & 2.70 \\
  & Periph-NF   & 8.0232 & 3.39  & 8.17  & 1.90 \\
  & Periph      & 8.1681 & 2.54  & 6.39  & 1.35 \\
  & STL-10       & 6.9973 & 9.55  & 18.96 & 7.43 \\
  & ImageNet-100 & 6.7985 & 10.77 & 21.07 & 8.71 \\
  & ImageNet-1K & 6.7964 & 10.74 & 21.08 & 8.77 \\
\midrule

\multirow{6}{*}{Places365}
  & Baseline    & 3.9690 & 25.63 & 51.90 & 23.16 \\
  & Fovea-Gaze  & 4.2347 & 21.86 & 46.21 & 19.14 \\
  & Periph-NF   & 4.2621 & 20.51 & 44.58 & 17.86 \\
  & Periph      & 4.2671 & 20.26 & 44.10 & 17.65 \\
  & STL-10       & 3.8281 & 26.57 & 53.47 & 24.82 \\
  & ImageNet-100 & 3.9207 & 24.99 & 51.21 & 23.32 \\
  & ImageNet-1K & 3.6264 & 30.17 & 58.46 & 28.36 \\
\bottomrule
\end{tabular}}

\end{table}
